Towards Instance-Optimal Offline Reinforcement Learning with Pessimism

We study the offline reinforcement learning (offline RL) problem, where the goal is to learn a reward-maximizing policy in an unknown Markov Decision Process (MDP) using the data coming from a policy $\mu$. In particular, we consider the sample complexity problems of offline RL for finite-horizon MDPs. Prior works study this problem based on different data-coverage assumptions, and their learning guarantees are expressed by the covering coefficients which lack the explicit characterization of system quantities. In this work, we analyze the Adaptive Pessimistic Value Iteration (APVI) algorithm and derive the suboptimality upper bound that nearly matches \[ O\left(\sum_{h=1}^H\sum_{s_h,a_h}d^{\pi^\star}_h(s_h,a_h)\sqrt{\frac{\mathrm{Var}_{P_{s_h,a_h}}{(V^\star_{h+1}+r_h)}}{d^\mu_h(s_h,a_h)}}\sqrt{\frac{1}{n}}\right). \] In complementary, we also prove a per-instance information-theoretical lower bound under the weak assumption that $d^\mu_h(s_h,a_h)>0$ if $d^{\pi^\star}_h(s_h,a_h)>0$. Different from the previous minimax lower bounds, the per-instance lower bound (via local minimaxity) is a much stronger criterion as it applies to individual instances separately. Here $\pi^\star$ is a optimal policy, $\mu$ is the behavior policy and $d_h^\mu$ is the marginal state-action probability. We call the above equation the intrinsic offline reinforcement learning bound since it directly implies all the existing optimal results: minimax rate under uniform data-coverage assumption, horizon-free setting, single policy concentrability, and the tight problem-dependent results. Later, we extend the result to the assumption-free regime (where we make no assumption on $ \mu$) and obtain the assumption-free intrinsic bound. Due to its generic form, we believe the intrinsic bound could help illuminate what makes a specific problem hard and reveal the fundamental challenges in offline RL.

==> sections/application.tex <==
% !TEX root = ../characterize_ope.tex

\section{Applications: offline Task-agnostic and offline Reward-free learning}\label{sec:application}

From Corollary~\ref{cor:opt_offline}, our model-based offline learning algorithm has two steps: 1. constructing offline empirical MDP $\widehat{M}$ using the offline dataset {$\mathcal{D}=\{(s_{t}^{(i)}, a_{t}^{(i)}, r(s_{t}^{(i)}, a_{t}^{(i)}), s_{t+1}^{(i)})\}_{i \in[n]}^{t \in[H]}$}; 2. performing any accurate black-box \emph{planning} algorithm and returning $\widehat{\pi}^\star$(or $\widehat{\pi}$) as the final output. However, the only \emph{effective} data (data that contains stochasticity) is $\mathcal{D}'=\{(s_{t}^{(i)}, a_{t}^{(i)})\}_{i \in[n]}^{t \in[H]}$. This indicates we are essentially using the state-action space exploration data $\mathcal{D}'$ to solve the task-specific problem with reward $r$. With this perspective in mind, it is natural to ask: given only the offline exploration data $\mathcal{D}'$, can we efficiently learn a set of potentially conflicting $K$ tasks ($K$ rewards) simultaneously? Even more, can we efficiently learn all tasks (any reward) simultaneously? This brings up the following definitions.
\vspace{1em}
\begin{definition}[Offline Task-agnostic Learning]\label{def:offline_ta}
	Given a offline exploration datatset $\mathcal{D}'=\{(s_{t}^{(i)}, a_{t}^{(i)})\}_{i \in[n]}^{t \in[H]}$ by $\mu$ with $n$ episodes. Given $K$ tasks with reward $\{r_k\}_{k=1}^K$ and the corresponding $K$ MDPs $M_k=(\mathcal{S}, \mathcal{A}, P, r_k, H, d_1)$. Can we use $\mathcal{D}'$ to output $\hat{\pi}_1,\ldots,\hat{\pi}_K$ such that 
	\[
	\P\left[\forall r_k,k\in[K], \norm{V^\star_{1,M_k}-V^{\hat{\pi}_k}_{1,M_k}}_\infty\leq\epsilon\right]\geq 1-\delta?
	\]
\end{definition}
\begin{definition}[Offline Reward-free Learning]\label{def:offline_rf}
	Given a offline exploration datatset $\mathcal{D}'=\{(s_{t}^{(i)}, a_{t}^{(i)})\}_{i \in[n]}^{t \in[H]}$ by $\mu$ with $n$ episodes. For any reward $r$ and the corresponding MDP $M=(\mathcal{S}, \mathcal{A}, P, r, H, d_1)$. Can we use $\mathcal{D}'$ to output $\hat{\pi}$ such that 
	\[
	\P\left[\forall r, \norm{V^\star_{1,M}-V^{\hat{\pi}}_{1,M}}_\infty\leq\epsilon\right]\geq 1-\delta?
	\]
\end{definition}
Definition~\ref{def:offline_ta} and Definition~\ref{def:offline_rf} are the offline counterparts of \citet{zhang2020task} and \citet{jin2020reward} in online RL. Those settings are of practical interests in the offline regime as well since in practice reward functions are often iteratively engineered to encourage desired behavior via trial and error and using one shot of offline exploration data $\mathcal{D}'$ to tackle problems with different reward functions could help improve sample efficiency. 

Our singleton absorbing MDP technique adapts to those settings and we have the following two theorems. The proofs of Theorem~\ref{thm:offline_ta}, \ref{thm:offline_rf} can be found in Appendix~\ref{sec:proof_ta}, \ref{sec:proof_rf}.
\vspace{1em}
 \begin{theorem}[optimal offline task-agnostic learning]\label{thm:offline_ta}
 	Given $\mathcal{D}'=\{(s_{t}^{(i)}, a_{t}^{(i)})\}_{i \in[n]}^{t \in[H]}$ by $\mu$. Given $K$ tasks with reward $\{r_k\}_{k=1}^K$ and the corresponding $K$ MDPs $M_k=(\mathcal{S}, \mathcal{A}, P, r_k, H, d_1)$. Denote $\iota=\log(HSA/\delta)$. Let $\widehat{\pi}_k^{\star}:=\operatorname{argmax}_{\pi} \widehat{V}_{1,M_k}^{\pi}$ $\forall k\in[K]$, when $n>O(H\cdot[\iota+\log(K)]/d_m)$, then with probability $1-\delta$,
 	\[
 	\norm{V_{1,M_k}^\star-V_{1,M_k}^{\widehat{\pi}_k^{\star}}}_\infty\leq 
 	O\left[\sqrt{\frac{H^2 (\iota+\log(K))}{n d_m}}+\frac{H^{2.5}S^{0.5}(\iota+\log(K))}{nd_m}\right].
 	\;\;\forall k\in[K]
 	\]
 \end{theorem}

\begin{theorem}[optimal offline reward-free learning]\label{thm:offline_rf}
	Given $\mathcal{D}'=\{(s_{t}^{(i)}, a_{t}^{(i)})\}_{i \in[n]}^{t \in[H]}$ by $\mu$. For any reward $r$ denote the corresponding MDP $M=(\mathcal{S}, \mathcal{A}, P, r, H, d_1)$. Denote $\iota=\log(HSA/\delta)$. Let $\widehat{\pi}^{\star}_M:=\operatorname{argmax}_{\pi} \widehat{V}_{1,M}^{\pi}$ $\forall r$, when $n>O(HS\cdot\iota/d_m)$, then with probability $1-\delta$, 
	\[
	\norm{V_{1,M}^\star-V_{1,M}^{\widehat{\pi}^{\star}_M}}_\infty\leq O\left[\sqrt{\frac{H^2S \cdot\iota}{n d_m}}+\frac{H^{2}S\cdot\iota}{nd_m}\right].
	\;\;\forall r,M.
	\]
\end{theorem}

By a direct translation of both theorems, we have sample complexity of order $\widetilde{O}(H^2\log(K)/d_m\epsilon^2)$ and $\widetilde{O}(H^2S/d_m\epsilon^2)$. All the parameters have the optimal rates, see lower bound in \citet{zhang2020task} and \citet{jin2020reward}. In particular, the higher order dependence in Theorem~\ref{thm:offline_rf} is also tight. 





































%\newpage

==> sections/discussion.tex <==
% !TEX root = ../characterize_ope.tex


\noindent\textbf{Unifying different offline settings.}
This work solves the sample optimality problems for local uniform OPE, offline task-agnostic and offline reward-free problems. If we take a deeper look, the algorithmic frameworks utilized are all based on model-based empirical MDP construction and planning. Therefore, as long as we can analyze such framework sharply (\emph{e.g.} via absorbing-MDP type trick), then it is hopeful that our techniques can be generalized to more sophisticated settings. On the other hand, things could be more tricky for online RL since exploration phases need to be specifically designed for each settings and there may not be one general algorithmic pattern that dominates. Our findings reveal model-based framework is fundamental for offline RL as it subsumes settings like local uniform OPE, offline task-agnostic and offline reward-free into the identical learning pattern. Therefore, understanding model-based approaches is crucial for offline RL. 

\noindent\textbf{On the higher order error term.}
Our main result (Theorem~\ref{thm:optimal_upper_bound}) has an additional $\sqrt{HS}$ dependence in the higher order error term and we cannot further remove it based on our current technique. Moreover, suboptimal dependence in parameter $H,S$ in the higher order terms is a long-lasting issue in almost all state-of-the-art online RL algorithms (\emph{e.g.} \citet{azar2017minimax,jin2018q,dann2019policy,zhang2020reinforcement}). How to obtain optimality not only for the main term but also for the higher order error terms remains elusive for the community.



\noindent\textbf{Uniform OPE and beyond.}
The current study of uniform OPE derives results with expression using parameter dependence which lacks the characterization of each individual policy. Deriving instance-dependent uniform convergence result will draw a clearer picture on the individual behaviors for each policy. Besides, this work concentrates on Tabular MDPs and generalizing uniform convergence to more practical settings like linear MDPs, game environments and multi-agent settings are promising future directions.  Specifically, general complexity measure (mirroring VC-dimensions and Rademacher complexities for statistical learning problems) that precisely captures local and global uniform convergence beyond the tabular cases would be of great interest.  

%It remains unclear whether the lower bound can be achieved for the global policy class in uniform OPE. We conjecture that this is true but it will require some new techniques. %Moreover, offline tabular setting is only a starting point and extending the setting to linear MDPs, kernel spaces and function approximation to combine model-based methods would be more practical and helpful for offline learning in general.  




%\yw{We have already discussed the relationship with simulation lemma and Duan et al earlier.}
%\textbf{The pointwise OPE analysis as refined simulation lemma.}
%One intrinsic challenge for sequential decision making problem is decisions made over long horizon may become imprecise due to the error propagation. Therefore, accurate planning over long horizon is core for the success of RL and getting optimal dependence on $H$ is highly non-trivial, \emph{e.g.} see COLT open problem \citep{jiang2018open}. How much improvement/novelty does our analysis made in this task? For example, the standard analysis tool for model-based estimates is \emph{simulation lemma} \citep{jiang2018notes,kearns2002near}, it follows (assuming deterministic reward):\footnote{For detailed verification of the computation, see Appendix~\ref{sec:app_sl}.}
%{\small
%\begin{align*}
%\norm{\widehat{v}^\pi-v^\pi}_\infty&\leq H^2 \sup_{t,s_t,a_t}\norm{\widehat{P}(\cdot|s_t,a_t)-P(\cdot|s_t,a_t)}_1\\
%&\leq O\left(\sqrt{\frac{H^4S^2\log(HSA/\delta)}{nd_m}}\right),
%\end{align*}
%}which has provable complexity of $\widetilde{O}(H^4S^2/d_m\epsilon^2)$. Meanwhile, our Lemma~\ref{thm:single_finer_bound} only has order $\widetilde{O}(H^2/d_m\epsilon^2)$, which has $H^2S^2$ improvement over the vanilla \emph{simulation lemma}. Moreover, this result essentially matches the Corollary~1 of \cite{duan2020minimax} and is minimax optimal under our Assumption~\ref{assume2} (our $d_m=\min_{s,a} \bar{\mu}_h(s,a)$ in their case). Our analysis reveals direct model-based plug-in estimator is tight, which helps to correct the commonly held misunderstanding that purely model plug-in estimator can only provide loose bound due to \emph{simulation lemma}. 


%\textbf{Comparison to $\widetilde{O}(H^3S^2A/\epsilon^2)$ uniform convergence bound in \citet{yin2020asymptotically} (Section~3.2).} Their results require number of episodes in each splitted data $M$ to satisfy $\widetilde{O}(\sqrt{nSA})>M>O(HSA)$. To achieve data efficiency, they need $n\approx \Theta(H^2SA/\epsilon^2)$ and by that condition $M$ has to satisfy $M\approx C\cdot HSA$. In this case, data-splitting version needs to create $N=n/M$ empirical transition dynamics and each dynamics use $H^3/N\approx C\cdot H^2SA/\epsilon^2$ episodes which is less than the lower bound ($O(H^3)$) required for learning. Also, it has $N$ empirical transitions so it is not clear which transition to plan over. Analysis for OPEMA completely avoids these issues (See those algorithms in Section~\ref{sec:alg}). 




==> sections/method.tex <==

% !TEX root = ../Uniform_OPE_icml.tex

\subsection{Tabular Marginalized Importance Sampling Estimator}

\textbf{We stick with the tabular marginalized importance sampling estimator (TMIS). }

In addition to the non-stationary, finite horizon tabular MDP $M=(\mathcal{S},\mathcal{A},r,T,d_1,H)$ (where $S:=|\mathcal{S}|<\infty$ and $A:=|\mathcal{A}|<\infty$), non-stationary logging policy $\mu$ and target policy $\pi$ in Section~\ref{sec:preliminary}, we denote $d^\mu_t(s_t,a_t)$ and $d^\pi_t(s_t,a_t)$ the induced joint state-action distribution at time $t$ and the state distribution counterparts $d^\mu_t(s_t)$ and $d^\pi_t(s_t)$, satisfying $d^{\pi}_t(s_t,a_t)=d^{\pi}_t(s_t)\cdot \pi(a_t|s_t)$.\footnote{For $\mu$, $d^{\mu}_t(s_t,a_t)=d^{\mu}_t(s_t)\cdot \mu(a_t|s_t)$.} The initial distributions are identical $d_1^\mu=d^\pi_1=d_1$. Moreover, we use $P^\pi_{i,j}\in\mathbb{R}^{S\times S}, \;\forall j<i$ to represent the state transition probability from step $j$ to step $i$ under policy $\pi$, where $P^\pi_{t+1,t}(s^\prime|s)=\sum_a P_{t+1,t}(s^\prime|s,a)\pi_t(a|s)$.  The marginal state distribution vector ${d}_t^\pi(\cdot)$ satisfies
${d}_t^\pi  = {P}^{\pi}_{t,t-1} {d}_{t-1}^\pi,$

Historical data $\mathcal{D}=\left\lbrace (s_t^{(i)},a_t^{(i)},r_t^{(i)})\right\rbrace_{i\in[n]}^{t\in[H]} $ was obtained by logging policy $\mu$ and we can only use $\mathcal{D}$ to estimate the value of target policy $\pi$, \emph{i.e.} $v^\pi$. Suppose we only assume knowledge about $\pi(a|s)$ for all $(s,a)\in\mathcal{S}\times\mathcal{A}$ and \emph{do not observe} $r_t(s_t,a_t)$ for any actions other than the noisy immediate reward $r_t^{(i)}$ after observing $s_t^{(i)},a_t^{(i)}$. 

\begin{assumption}[Bounded rewards]\label{assume1}
	 $\forall \;t=1,...,H$ and $i=1,...,n$, $0\leq r^{(i)}_t\leq R_{\max}$.
\end{assumption}
The bounded reward assumption can be relaxed to:  $\exists R_{\max},\sigma<+\infty$ such that $0\leq \mathbb{E}[r_t|s_t,a_t,s_{t+1}]\leq R_{\max}$, $\mathrm{Var}[r_t|s_t,a_t,s_{t+1}]\leq \sigma^2$ (as in \citet{xie2019towards}), for achieving Cramer-Rao lower bound. However, the boundedness will become essential for applying concentrate inequalities in deriving high probability bounds.

\begin{assumption}\label{assume2}
	Logging policy $\mu$ obeys $d_m:=\min_{t,s_t}d^\mu_t(s_t)>0$.
\end{assumption}
This assumption is always required for the consistency of off-policy evaluation estimator. 

\begin{assumption}[Bounded weights]\label{assume3}
	$\tau_s:=\max_{t,s_t}\frac{d^\pi_t(s_t)}{d^\mu_t(s_t)}<+\infty$ and $\tau_a:=\max_{t,s_t,a_t}\frac{\pi(a_t|s_t)}{\mu(a_t|s_t)}<+\infty$.
\end{assumption}
Assumption~\ref{assume3} is also necessary for discrete state and actions, as otherwise the second moments of the importance weight would be unbounded and the MSE of estimators will become intractable . The bound on $\tau_s$ is natural since $\tau_s\leq \max_{t,s_t}\frac{1}{d^\mu_t(s_t)}=\frac{1}{\min_{t,s_t}d^\mu_t(s_t)}=\frac{1}{d_m}$ and it's finite by the Assumption~\ref{assume2}; similarly, $\tau_a<\infty$ is also automatically satisfied if $\min_{t,s_t,a_t}\mu(a_t|s_t)>0$.  

\subsection{Tabular-MIS estimator}

Marginalized importance sampling directly estimates
the marginalized state visitation distribution $\widehat{d}_t$ and defines the MIS estimator:

\begin{equation}\label{MIS_def}
\widehat{v}^\pi_{MIS} =\frac{1}{n}\sum_{i=1}^n\sum_{t=1}^H\frac{\widehat{d}^\pi_t(s_t^{(i)})}{\widehat{d}^\mu_t(s^{(i)}_t)}\widehat{r}^\pi_t(s^{(i)}).
\end{equation}
and $\widehat{d}^\mu_t(\cdot)$ is directly estimated using the empirical mean, \emph{i.e.} $\widehat{d}^\mu_t(s_t):=\frac{1}{n}\sum_i \mathbf{1}(s_t^{(i)}=s_t):=\frac{n_{s_t}}{n}$ whenever $n_{s_t}>0$ and $\widehat{d}^\pi_t(s_t)/\widehat{d}^\mu_t(s_t)=0$ when $n_{s_t}=0$. Then the MIS estimator \eqref{MIS_def} becomes:
\begin{equation}\label{MIS}
\widehat{v}^\pi_{MIS}=\sum_{t=1}^H\sum_{s_t}\widehat{d}^\pi_t(s_t)\widehat{r}^\pi_t(s_t)
\end{equation}

\paragraph{Construction of \TMIS .} 
  
We can construct empirical estimates for $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})$ and $\widehat{r}_t(s_t,a_t)$ as: 
{\small
\begin{equation}\label{eq:tabular_MIS_construction}
%\hspace{-3.5mm}
\begin{aligned}
\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})&=\frac{\sum_{i=1}^n\mathbf{1}[(s^{(i)}_{t+1},a^{(i)}_t,s^{(i)}_t)=(s_{t+1},s_{t},a_{t})]}{n_{s_{t},a_{t}}}\\
\widehat{r}_t(s_t,a_t)&=\frac{\sum_{i=1}^n r_t^{(i)}\mathbf{1}[(s^{(i)}_t,a^{(i)}_t)=(s_t,a_t)]}{n_{s_t,a_t}},\\
\end{aligned}
\end{equation}
}
where we set $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})=0$ and $\widehat{r}_t(s_t,a_t)=0$ if $n_{s_t,a_t}=0$, with $n_{s_t,a_t}$ the empirical visitation frequency to state-action $(s_t,a_t)$ at time $t$. The corresponding estimation of $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})$ and $\widehat{r}_t(s_t,a_t)$ are defined as:

\begin{equation}\label{eq:tabular_MIS_construction2}
\begin{aligned}
\widehat{P}^\pi_t(s_t|&s_{t-1})=\sum_{a_{t-1}}\widehat{P}_t(s_t|s_{t-1},a_{t-1})\pi(a_{t-1}|s_{t-1}),\\
\widehat{r}^\pi_t(s_t)&=\sum_{a_t}\widehat{r}_t(s_t,a_t)\pi(a_t|s_t),\;\widehat{d}^\pi_t=\widehat{P}^\pi_t\widehat{d}^\pi_{t-1}. 
\end{aligned}
\end{equation}




%\red{However, model-based approaches are not well-understood even in tabular setting.  Some discussions and summary of the understanding of tabular methods are here: \url{http://nanjiang.cs.illinois.edu/files/cs598/note3.pdf}
%In particular, check the "Simulation Lemma", and check out the various ``naive approaches'' to analyze the model-based methods.}



==> sections/offline.tex <==
% !TEX root = ../Uniform_convergence_OPE.tex 
%Why do we care about above statistical learning theories? Most critically, Uniform OPE provides theoretical foundation for efficient \emph{offline learning} algorithm.




In this section we discuss the implication of our results on offline learning. As we discussed earlier in the introduction, a uniform OPE bound of $\epsilon$ implies that the corresponding ERM algorithm finds a $2\epsilon$-suboptimal policy.  But it also implies that all other offline policy-learning algorithms that are not ERM, we could gracefully decompose their error into optimization error and statistical  (generalization) error. 
\begin{theorem}\label{thm:offlinelearning}
	Let $\hat{\pi}^* = \argmax_{\pi} \hat{v}^{\pi}$ --- the empirically optimal policy. Let $\hat{\pi}$ be any data-dependent choice of policy such that $\hat{v}^{\hat{\pi}^*} - \hat{v}^{\hat{\pi}} \leq \epsilon_\text{opt}$, then. There is a universal constant $c$ such that w.p. $\geq 1-\delta$ 
	\begin{enumerate}
		\itemsep1pt
		\item 	$
		v^{\pi^*}  - v^{\hat{\pi}} \leq c\sqrt{\frac{H^4S\log(HSA/\delta)}{d_m \cdot n}} + \epsilon_\text{opt}.
		$
		\item If  $\delta< e^{-S}$, the bound improves to $c\sqrt{\frac{H^4S\log(HSA/\delta)}{d_m \cdot n}} +  \epsilon_\text{opt}$. And if in addition $\hat{\pi}$ is deterministic, the bound further improves to 
		$c\sqrt{\frac{H^3\min\{H,S\}\log(HSA/\delta)}{d_m \cdot n}} +  \epsilon_\text{opt}$.
		\item If $\epsilon_\text{opt}\leq \sqrt{H}/S$ and that 
		$||\widehat{V}^{\hat{\pi}}_t-\widehat{V}^{\widehat{\pi}^\star}_t ||_\infty\leq\epsilon_\text{opt},\;\forall t=1,...,H$
		%	$||\widehat{Q}^{\hpi}_1-\widehat{Q}^{\widehat{\pi}^\star}_1 ||_\infty\leq\epsilon_\text{opt} \;\forall t=2,...,H$
		, then 
		$
		v^{\pi^*}  - v^{\hat{\pi}} \leq c\sqrt{\frac{H^3\log(HSA/\delta)}{d_m \cdot n}} + \epsilon_\text{opt}.
		$
	\end{enumerate}
\end{theorem}

\begin{table*}
	\caption{A comparison of related offline policy learning results. }
	\label{table}
	\centering
	\resizebox{\linewidth}{!}{%
		\begin{tabular}{llll}
			\toprule
			%\multicolumn{2}{c}{Part}                   \\
			\cmidrule(r){1-3}
			Method/Analysis     &Setting& Guarantee     & Sample complexity$^b$ \\
			\midrule
			\cite{agarwal2020model} &Generative model &$\epsilon+O(\epsilon_{\text{opt}}/(1-\gamma))$-optimal  & {$\widetilde{O}(SA/(1-\gamma)^3 \epsilon^2)$}    \\
			\cite{le2019batch,chen2019information} &$\infty$-horizon offline & $\epsilon$-optimal policy  & $\widetilde{O}((1-\gamma)^{-6}C_\mu/ \epsilon^2)$   \\
			\cite{xie2020q} & $\infty$-horizon offline & $\epsilon$-optimal policy  & $\widetilde{O}((1-\gamma)^{-4}C_\mu/ \epsilon^2)$   \\
			{SIMPLEX} for exact empirical optimal$^a$ & $H$-horizon offline  &$\epsilon$-optimal policy & \mypink{$\widetilde{O}(H^3/d_m \epsilon^2)$}    \\
			{PI/VI} for $\epsilon_{\text{opt}}$-empirical optimal  &$H$-horizon offline   & $(\epsilon+\epsilon_{\text{opt}})$-optimal policy & \mypink{$\widetilde{O}(H^3/d_m \epsilon^2)$}    \\
			Minimax lower bound (Theorem~\ref{thm:learn_low_bound})  &$H$-horizon offline    & over class $\mathcal{M}_{d_m}$     & $\Omega(H^3/d_m\epsilon^2)$  \\
			\bottomrule
		\end{tabular}
	}
	\hspace{-4cm}\footnotesize{ $^a$ PI/VI or SIMPLEX is not essential and can be replaced by any efficient empirical MDP solver.}\\
	
	\footnotesize{ $^b$ \emph{Episode} complexity in $H$-horizon setting is comparable to \emph{step} complexity in $\infty$-horizon setting because our finite-horizon MDP is \emph{time-inhomogeneous}.  Informally, we can just take $(1-\gamma)^{-1} \asymp H$ and $C_\mu\asymp 1/d_m$. }
\end{table*}

The third statement implies that all sufficiently accurate planning algorithms based on the empirically estimated MDP are optimal. For example, we can run value iteration or policy iteration to the point that $\epsilon_{\text{opt}} \leq O(H^3/{n d_m})$.  

\noindent\textbf{Comparing to existing work.} Previously no algorithm is known to achieve the optimal sample complexity in the offline setting. Our result also applies to the related generative model setting by replacing $1/d_m$ with $SA$, which avoids the data-splitting procedure usually encountered by specific algorithm design \citep[e.g.,][]{sidford2018near}. 
The analogous policy-learning results In the generative model setting \citep[Theorem 1]{agarwal2020model} , 
 %This analysis has an improvement over \cite{agarwal2020model} as they have a
 achieves a suboptimality of $\tilde{O}(  (1-\gamma)^{-3}SA/n + (1-\gamma)^{-1} \epsilon_{\text{opt}}  )$ with no additional assumption on $ \epsilon_{\text{opt}}$. Informally, if we replace $(1-\gamma)^{-1}$ with $H$, then our result improves the bound from $H \epsilon_{\text{opt}}$ to just $\epsilon_{\text{opt}}$ for $\epsilon_{\text{opt}}\leq \sqrt{H}/S$. 
  %$O(\epsilon_{\text{opt}}/(1-\gamma))$ term which should be translated as $O(\epsilon_{\text{opt}}H)$ in the finite horizon setting. 
  These results are summarized in Table~\ref{table}. 
  
  \noindent\textbf{Sparse MDP estimate.}
  We highlight that the result does not require the estimated MDP to be an accurate approximation in any sense. Recall that the true MDP has $O(S^2)$ parameters (ignoring the dependence on $H,A$ and logarithmic terms), but our result is valid provided that  $n = \tilde{\Omega}(1/d_m)$ which is $\Omega(S)$. This suggests that we may not even exhaustively visit all pairs to state-transitions and that the estimator of $\hat{P}_t$ is allowed to be zero in many coordinates.
  
  
  \noindent\textbf{Optimal computational complexity.}
  Lastly, from the computational perspective, we can leverage the best existing solutions for solving optimization $\widehat{\pi}^\star:=\text{argmax}_{\pi\in\Pi} \widehat{v}^\pi$. For example, with $\epsilon_{\text{opt}}>0$, as explained by \citet{agarwal2020model}, value iteration ends in $O(H\log \epsilon_{\text{opt}}^{-1})$ iteration 
  and takes at most $O(HSA)$ time after the model has been estimated with one pass of the data ($O(nH)$ time). We have a total computational complexity of $O(H^4/(d_m \epsilon^2) + H^2SA\log(1/\epsilon))$ time algorithm for obtaining the $\epsilon$-suboptimal policy using $n=O(H^4/(d_m \epsilon^2) $ episodes. This is essentially optimal because the leading term $H^4SA/\epsilon^2$ is required even to just process the data needed for the result to be information-theoretically possible. In comparison, the algorithm that obtains an exact empirical optimal policy $\widehat{\pi}^\star$, the SIMPLEX policy iteration runs in time $O(\text{poly}(H,S,A,n))$ \citep{ye2011simplex}. 
 





% When uniform convergence in OPE is guaranteed, we can derive offline learning algorithms in a straightforward way by learning the empirical optimal policy $\widehat{\pi}^\star:=\text{argmax}_{\pi\in\Pi} \widehat{v}^\pi$. As a result, model-based Uniform OPE allows the use of \emph{any} efficient planning algorithm in the empirical MDP, which simplifies algorithm design, as the algorithm utilized need not be tied to the sampling procedure/offline data $\mathcal{D}$. Also, it avoids the data-splitting procedure usually encountered by specific algorithm design, \emph{e.g.} \cite{sidford2018near}. Formally, by leveraging the global Uniform OPE result we have the following:
%
%\begin{theorem}[Offline learning algorithm]\label{thm:offline_learn}
%	Suppose a model-based OPE method $\widehat{v}$ achieves $\epsilon_{\text{uni}}$-uniform convergence, \textit{i.e.} with high probability, $\sup_{\pi\in\Pi} \left|\widehat{v}^\pi-v^\pi\right|\leq \epsilon_{\text{uni}}$. Assuming the realizability that $\pi^\star\in\Pi$. Then by selecting $\widehat{\pi}^\star:=\text{argmax}_{\pi\in\Pi} \widehat{v}^\pi$, we obtain with high probability, $
%	v^{\pi^\star}-v^{\widehat{\pi}^\star}\leq 2\epsilon_{\text{uni}}.
%	$ In particular, with OPEMA, if apply Thm~\ref{thm:thre}, then $\widehat{\pi}^\star$ is $\widetilde{O}(\sqrt{H^4S/nd_m})$-optimal policy and if apply Thm~\ref{thm:finer_bound} we know $\widehat{\pi}^\star$ is essentially tighter $\widetilde{O}(\sqrt{H^3S/nd_m})$-optimal policy, regardless of the planning algorithm. 
%\end{theorem}
%The proof was explained in the motivation section before. If $|\Pi|$ is relatively small, we can find $\widehat{\pi}^\star$ with direct policy search: we traverse all the policies $\pi\in\Pi$ and calculate $\widehat{v}^\pi$, and learn the empirical optimal policy $\widehat{\pi}^\star$. If $|\Pi|$ is large, then $\widehat{\pi}^\star:=\text{argmax}_{\pi\in\Pi} \widehat{v}^\pi$ can be solved efficiently by applying standard Policy Iteration (PI) or Value Iteration (VI) on empirical MDP $\widehat{M}$ \citep{sutton2018reinforcement} since $\widehat{M}$ is known. Theorem~\ref{thm:finer_bound} guarantees offline learning with complexity $\widetilde{O}(H^3S/d_m\epsilon^2)$ is one factor away from optimality in learning context (see Theorem~\ref{thm:learn_low_bound} in appendix). 
%
%Theorem~\ref{thm:offline_learn} requires at least one optimal policy to be within the class for the result to work. In contrast, the local uniform convergence result in Theorem~\ref{thm:local_uni_opt} guarantees a $O(\epsilon_{\text{opt}}+\epsilon)$-optimal policy for any policy $\pi$ in the neighborhood of $\widehat{\pi}^\star$ without requirement for optimal policy. Formally, we have the following:
%
%\begin{theorem}\label{thm:uni_opt_local}
%	Suppose $\epsilon_{\text{opt}}\leq \sqrt{H}/S$ and $\widehat{\pi}$ satisfies $||\widehat{Q}^{\hpi}_1-\widehat{Q}^{\widehat{\pi}^\star}_1 ||_\infty\leq\epsilon_\text{opt}$ and $
%	||\widehat{V}^{\hpi}_t-\widehat{V}^{\widehat{\pi}^\star}_t ||_\infty\leq\epsilon_\text{opt},\;\forall t=2,...,H
%	$. There exists constant $c_1,c_2$ such that when $n>c_1H^3\log(HSA/\delta)/d_m\epsilon^2$ with probability $1-\delta$,
%{\small	\[
%	{Q}^{\pi^\star}_1-{Q}_1^{\widehat{\pi}}\leq c_2\cdot \epsilon\cdot\mathbf{1}+\epsilon_{\text{opt}}\cdot\mathbf{1}.
%	\]}
%\end{theorem}
%In the case where $\epsilon_{\text{opt}}=0$, we have $\widehat{\pi}=\widehat{\pi}^\star$ achieves the optimal sample complexity $O(H^3\log(HSA/\delta)/d_m\epsilon^2)$. 







%\twocolumn[text]

==> sections/simulation.tex <==
% !TEX root = ../Uniform_convergence_OPE.tex




%\yub{Maybe ``Proof overview'' as the subtitle?}
In this section we use a simple simulated environment to empirically demonstrate the correct scaling in $H$. Direct evaluating $\sup_{\pi\in\Pi} |\widehat{v}^\pi-v^\pi|$ empirically is computationally infeasible since the policy classes we considered here contains either $A^{HS}$ or $\infty$ many policies. 
%For example, if we pick $K$ policies inside the policy class to numerically verify and $K\ll A^{HS}$, then by Lemma~\ref{thm:single_finer_bound} and a union bound, the sup over all $K$ policies is still of order $\widetilde{O}(H^2\log(K))$ (instead of the correct lower bound $\Omega(H^3)$ in Thm~\ref{thm:uni_lower}). 
%To address this issue, 
Instead, in the experiment we will plot the sub-optimality gap $ |v^\star-v^{\widehat{\pi}^\star}|$ with $\hat{\pi}^\star$ being the outputs of policy planning algorithms. The sub-optimality gap is considered as a surrogate for the lower bound of $\sup_{\pi\in\Pi} |\widehat{v}^\pi-v^\pi|$.
%use the learning result and measure $|v^\star-v^{\widehat{\pi}^\star}|$ as a surrogate for $\sup_{\pi\in\Pi} |\widehat{v}^\pi-v^\pi|$. 
Concretely, the non-stationary MDP has $2$ states $s_0,s_1$ and $2$ actions $a_1,a_2$ where action $a_1$ has probability $1$ going back the current state and for action $a_2$, there is one state s.t. after choosing $a_2$ the dynamic transitions to both states with equal probability $\frac{1}{2}$ and the other one has asymmetric probability assignment ($\frac{1}{4}$ and $\frac{3}{4}$). The transition after choosing $a_2$ is changing over different time steps therefore the MDP is non-stationary and the change is decided by a sequence of pseudo-random numbers (Figure~\ref{fig:mdp} shows the transition kernel at a particular time step). Moreover, to make the learning problem non-trivial we use non-stationary rewards with $4$ categories, \emph{i.e.} $r_t(s,a)\in\{\frac{1}{4},\frac{2}{4},\frac{3}{4},1\}$ and assignment of $r_t(s,a)$ for each value is changing over time (see Section~\ref{sec:simluation_detail} in appendix for more details). Lastly, the logging policy in Figure~\ref{fig:different_H} is uniform with $\mu_t(a_1|s)=\mu_t(a_2|s)=\frac{1}{2}$ for both states.


Figure~\ref{fig:different_H} use a fixed number of episodes $n=2048$ while varying $H$ to examine the horizon dependence for uniform OPE. We can see for fixed pointwise OPE with OPEMA (blue line), $|v^\pi-\widehat{v}^\pi|$ scales as $O(\sqrt{H^2})$ which reflects the bound of Lemma~\ref{thm:single_finer_bound}; for the model-based planning, we ran both VI and PI until they converge to the empirical optimal policy $\widehat{\pi}^\star$. %We run both VI/PI for sufficient iterations so they converge to the exact empirical optimal policy $\widehat{\pi}^\star$. 
The figure shows that for this MDP example $|v^\star-v^{\widehat{\pi}^\star}|$ scales as $O(\sqrt{H^3/d_m})$ for fixed $n$ since it is parallel to the reference magenta line. This fact empirically shows $O(\sqrt{H^3/d_m})$ bound is required %for both offline learning and UCOPE and 
confirms the scaling of our theoretical results. 
%For other related simulation %(\emph{e.g.} relative error $|v^\star-v^{\widehat{\pi}^\star}|/v^\star$ for checking experimental correctness), 
%see Appendix~\ref{sec:simluation_detail}.

\begin{figure}
	\centering     %%% not \center
	\subfigure[A non-stationary MDP]{\label{fig:mdp}\includegraphics[width=0.45\linewidth]{MDP-instance.pdf}}
	\subfigure[RMSE vs. Horizon $H$]{\label{fig:different_H}\includegraphics[width=0.5\linewidth]{verify_uniform_convergence.pdf}}
	\caption{Log-log plot  showing the dependence on horizon of uniform OPE and pointwise OPE via learning ($|{v}^{\star}-v^{\widehat{\pi}^\star}|$) over a non-stationary MDP example.}
	\label{fig:main}
\end{figure}


%\red{Talk about how CR lower bound might not be asymptotically achievable in some cases.}
